RASAECO: Requirements Analysis of Software for the AECO Industry

Digitalization is forging its path in the architecture, construction, engineering, operation (AECO) industry. This trend demands not only solutions for data governance but also sophisticated cyber-physical systems with a high variety of stakeholder background and very complex requirements. Existing approaches to general requirements engineering ignore the context of the AECO industry. This makes it harder for the software engineers usually lacking the knowledge of the industry context to elicit, analyze and structure the requirements and to effectively communicate with AECO professionals. To live up to that task, we present an approach and a tool for collecting AECO-specific software requirements with the aim to foster reuse and leverage domain knowledge. We introduce a common scenario space, propose a novel choice of an ubiquitous language well-suited for this particular industry and develop a systematic way to refine the scenario ontologies based on the exploration of the scenario space. The viability of our approach is demonstrated on an ontology of 20 practical scenarios from a large project aiming to develop a digital twin of a construction site.

==> 05o_experience_report_obsolete_parts.tex <==

\todo{dag}{
\begin{itemize}
    \item We need a clear case why "classical" requirements approaches did not work!
    \item Explain in more detail why post-its didn't work
    \item Explain the iDEF0 approach (diagrams, then requirements list) and compare in more detail
        why our approach is better.
    \item See how~\cite{dronology} covered analysis.
        This is what looks most promising to me (mristin).
        Mind that they~\cite{dronology} did not use any data and also no clear criteria!
        Maybe that's the best approach?
    \item Otherwise, use~\cite{glinz_scenarios} or~\cite{lightweight_requirements_assesments} as
        criteria? (mristin: I like~\cite{glinz_scenarios} more.)
        Can we really get any meaningful data to back up our claims?
    \item Compare again how~\cite{arayici} and~\cite{bim_governance} did the requirements.
    \item See also what some of \texttt{re\_in\_*} papers did (see the \texttt{bibliography.bib}).
\end{itemize}
}

We evaluated our approach on a set of \todo{dag/mristin}{???} practical AECO scenarios arising from
industrial partners participating in the BIMprove project~\cite{bimprove}.
The scenarios were all elaborated in a group of 2 AECO professionals, 1 software engineer and
1 robotic engineer during a series of workshop sessions (\todo{dag/mristin}{???} note how long
the sessions took).

\textit{Two external engineers (non-AECO professionals) evaluated the scenarios using the following }
criteria (designed according to~\cite{glinz_scenarios}):
\begin{itemize}
    \item Adequacy of the scenario space (how well could the scenarios be represented in the 
        predefined three dimensions; how easy would it be to come up with a more suitable set of 
        dimensions)
    \item Readability of the document (how easy was it to comprehend; how much did pseudocode help
        and how much it made reading difficult),
    \item Verifiability of the scenario (how easy is it to test if the scenario has been implemented\
        correctly, not necessarily automatically),
    \item Modifiability of the scenarios (how easy would it be to change the scenario), and
    \item Reuse across the scenarios (how much sense did it make to reuse parts of the scenarios
        and structure them in an ontology).
\end{itemize}

Given the small number of participants, we asked the evaluators to give qualitative answers instead
of quantitative scores.
We assume that the quality of the requirements is a fair proxy of the quality of the approach and
assume further that a fallible approach would be reflected in bad requirements regardless of
the writers’ skill level and immediately evident from the qualitative answers.


==========


==========


\todo{dag}{??? Present the results.}

\todo{dag}{
Compare post-it session from the elicitation phase with the structured scenarios. Status: DONE

Discuss our experience -- what worked, what did not work. Status: DONE

Discuss how scenario space worked. Status: DONE.

Discuss how BIM worked as ubiquitous language. Status: DONE.

Discuss how ontology worked

Discuss whether we could "keep it simple"?

To read? To write? $\rightarrow$ writing markdown a bit too hard, but reading totally OK. Status: DONE

How did that compare to IDEF0 and the baseline? Status: DONE.

Could we live up to the expectation that we were more lightweight than BPMN, UML and IDEF0?

Could we live up to the expectation that the requirements were not fragmented?

Mention that tests played out well -- instead of disparate unit tests, we get more tests at the
integration/functional level --> we found those to be more valuable and changing less often,
similar to GORE.

Discuss the software tool

Discuss that we didn't use pseudo-code or structured text at all.
When we tried: a) the professionals were scared. b) writing EARS: too atomic, too long, hard to read.
}

\todo{dag}{From Wernher:
+ possible standardization

+ possible limits of this approach

+ enhancement of the SOA in AECO
}


==> 05oo_experience_report.tex <==
%234567890123456789012345678901234567890123456789012345678901234567890123456789012345678901234567890
\section{An Experience Report on Applying ANONYMIZED} \label{sec:evaluation}

% \todo{dag}{
% \begin{itemize}
%     \item Count approximately miro post-its and how many clusters; note down the clusters
%     ==> In total there were 9 clusters, in total they had 191 post-it notes. The number for each cluster is as follows:
% BIM Community	34
% Analysis	16
% Non-exisitng solutions	14
% Architecture requirements	30
% BIMprove project goals	28
% User stories	26
% User-devices and -interfaces	16
% BIMprove Scenarios	7
% UAV + Robots	20

%     \item Count the IDEF0 black boxes (how many ``black boxes''; reuse the term black box explicitly as it 
%         was already mentioned in the begining) ==> 23 black boxes
%     \item Count the number of resulting requirements from IDEF0 -- just a brief notice, but this is necessary
%         to give an impression on the order of magnitude ==> There were 188 requirements.
%     \item count the average number of words in the structured scenarios -- copy/paste text from HTML, 
%         give the minimal and maximal length and average.  ==> The average of the 12 scenarios was 904 words per scenario, minimum was 373 and maximum was 1930.
% \end{itemize}
% }

In this paper we have proposed a novel approach and a tool for eliciting, analyzing, specifying, 
and managing system scenarios in the AECO industries. 
We focused our efforts thus far on developing both the concepts and the tool to make them ready for
practical use.
Due to limited resources, we could not evaluate our approach on a set of different projects,
but the initial results look promising.
We recognize that more systematic field studies and varied use cases are needed to assess 
ANONYMIZED in a more rigorous manner.

We report our experience of applying our approach to writing structured system scenarios and 
compare our requirements analysis with the alternative approach based on 
IDEF0 ``black boxes''~\cite{idef0}.
The size of both the structured scenarios as well as the alternative requirements artifacts
% 18 = 12 original scenarios + 4 step scenarios + 2 risk management split in phases
using IDEF0 is modest (\emph{e.g.}, only 18 structured scenarios and 23 IDEF0 ``black boxes''),
so even internally in our project the number is too low to evaluate using any statistical method. 
Additionally there would be a statistical challenge in that we could not assume independence 
between the samples since every scenario is from the same project, ANONYMIZED~\cite{bimprove}. 
So our evaluation has to be qualitative.

\subsection{Our Requirements Analysis} \label{subsec:our-analysis}
We used our approach to write and structure system scenarios.
The process was lead by a software professional, who did the writing, as the AECO experts were 
clearly reluctant to do it.
However, the resulting markdown text was very readable and something they could comment and
approve.
We found it beneficial that the person doing the writing also was driving the meeting, 
because then the writer would steer the tempo of the discussion based on how quick it was possible to write 
structured text of good quality. 
Each of the sessions was about a specific topic (for instance, the scenario ``Truck Guidance'' 
as depicted in Table~\ref{tab:aspects}a), 
and what took place was something between an interview and a conversation.
In the end, we wrote 18 scenarios, where all scenarios were rather compact 
(between 373 and 1930 words, with 904 words per scenario on average).
In total, there were 15 sessions in the course of 3 weeks, each taking 2-2.5 hours. 

\subsection{Alternative: Branstorming + IDEF0} \label{subsec:alternative}
The alternative approach started with a brainstorming session.
All the stakeholders used the web-based tool Miro~\cite{MIRO} to elicit the requirements in form of 
short text snippets visualized as post-its.
The post-its were deduplicated and clustered by the participants (in total, 9 clusters and 191 post-its, 
where a cluster comprised between 7 and 34 post-its).
The links were drawn between the clusters and between the post-its to identify the (non-formal) relationships.
The participants then voted on the importance of each cluster (with 10 points assigned to each person) to
identify the priorities.
Finally, the weighted requirements were used as input for further analysis.

Each two participants were assigned a cluster of requirements for refinement.
For further analysis, we used IDEF0~\cite{idef0}, a method developed by U.S. Air Force and
widely used in many industries to model the functions, activities or processes of a system.
The approach is based on ``black box'' diagrams where the analysis starts with the most abstract
box, and descends into more details.
Each entity is described by a box with arrows representing inputs, outputs and controls, thus employing 
a simple and sparse graphical language.

Based on the graphical representation of the requirements, the participants wrote the requirements in natural language
as a table.
No explicit structure (\emph{e.g.}, AECO-specific context) was given, so the requirements could be freely
organized as the authors saw fit.
The teams responsible for the clusters organized freely as they pleased.
There were in total 23 ``black boxes'' resulting in 188 requirements.
The whole process took 3 weeks.

\subsection{Comparison} \label{subsec:comparison}

\textbf{Degree of participation}. 
The alternative approach was clearly more ``democratic'' as both brainstorming and IDEF0 require
little instruction and very little structure on the requirements analysis, so all could contribute 
directly.

In contrast, our approach forced a certain structure on the authors, so that they had to be at least
familiar with the relevant terms such as solution dimensions, definitions and data models.
Somewhat unexpectedly, thinking and writing in such structures proved to be too much of a barrier
for AECO experts, so a software professional had to take over that task.
The resulting text was very readable and something they could comment and finally approve,
but limited the free contributions by the remainder of the team.

\textbf{Discovering deeper issues}.
The relative free-form of the alternative approach delayed the positive confrontation
between what is easy/difficult to implement and what is of low/high value from an AECO
perspective.
The IDEF0 diagrams opened the ``black boxes'' only up to a point as
they were easy to draw and allowed the authors to focus on their particular problems, 
but also allowed them to ignore the different dimensions of the solution space.
This poses a major challenge since the authors did not dig deeper and missed to define and
understand key concepts and how they are linked.
For example, the requirements were often very focused, but ignored issues related to, 
\emph{e.g.}, mixing and lumping together different phases of the building lifecycle.

We experienced that our approach did not suffer from this problem as much as it framed our thinking 
substantially and forced us to think in the relations of solution space and references to 
definitions and data models.
Since the links between the scenarios \emph{had} to be specified also nudged the authors
to identify them in the first place.

\begin{figure}
    \begin{tabular}{p{0.1} p}
    a) & \includegraphics[scale=0.55]{tex/IDEF0_schedule_machinery.png} \\
    \noalign{\vskip 0.5cm}
    b) & 
        \begin{tabular}{p{0.1cm} p{7cm}}
            1. & Real-time position when on the construction-site \\
            2. & Map of entry, exit, and delivery points \\
            3. & Optimal and safest routes to locations \\
            4. & Information about blocked routes and areas \\
            5. & A list of contact persons at the site \\
            6. & Real-time schedule of suitable working hours, 
                 including entry and exit times, and working at delivery point \\
            7. & Delivery/work status and receive confirmation \\
            8. & Alerts of abnormal conditions and safety risks \\
            9. & Messaging to construction personnel for support
        \end{tabular}
    \end{tabular}
    \captionof{figure}{%
    \textbf{a)} IDEF0 ``black box'' for scheduling of subcontractors, actors and machinery,
    corresponding to the example in Table~\ref{tab:aspects}a).
    \textbf{b)} The respective requirements derived from the ``black box''.
    The authors indeed captured relevant requirements in b), but
    did not investigate deeper issues due to the lack of instruments to
    dissect scenarios along different dimensions.
    }
    \label{fig:IDEF0_schedule_machinery}
\end{figure}

Consider Figure~\ref{fig:IDEF0_schedule_machinery} describing requirements obtained by the alternative approach on the scenario ``Truck Guidance'' 
from Table~\ref{tab:aspects}a).
The authors indeed uncovered relevant requirements, but we believe that 
using structured scenarios provided better results.
The alternative requirements did not dig deeper as they lacked 
an instrument to dissect a scenario, say, along the aspects.
For example, why and how information is used was not included in 
the alternative requirements list~\ref{fig:IDEF0_schedule_machinery}b),
in particular the level of detail of the site maps, and if they are meant to
be machine readable, just visual navigation for the driver on a screen, or both.
In our structured scenarios these locations (entry, delivery location on site) are defined as \texttt{IfcZone} and available from the as-planned part of the scheduling module. 

Another example is that sub-requirements are more implicit such as requirement in Figure~\ref{fig:IDEF0_schedule_machinery}b)3. which mentions desired locations 
but does not specify how to obtain the related delivery or 
the responsible person for the reception.
In our structured scenario, we specify that this information is obtained 
from  ``scheduling system'' and that the ``planner role'' is responsible for
keeping it up-to-date.

Yet another example is that the ``black box'' scenario missed the analytics of 
matches between as-planned and as-observed, an important aspect of the system.
Thinking about how to measure and contrast this is very helpful when defining the need for data, and this was explicitly captured in our structured scenarios 
beneath the aspect section ``Analytics''.

\textbf{Bringing to light AECO-specific complexities}.
We often faced a challenge that since construction site activity is very complex and heterogeneous 
between construction projects, at some occasions the AECO experts had to consult with other colleagues 
to get some smaller (but important!) details clarified.
We observed that this happened more often with our approach than with the alternative. 
In the IDEF0 work the authors observed this only once, but with the Structured Scenarios this happened 2 times in one scenario and 3 times in another. 

For example, when we wrote a scenario on cost tracking (see Table~\ref{tab:aspects}c), 
we discussed how costs were estimated for certain operations.
Though a very knowledgeable AECO expert could answer many questions,
the method lead us to discuss details about the data flow, and he realized
only then that further consultations with his AECO colleagues are necessary instead
of giving us a generic answer.
For us this indicates that our method is better suited to drilling down 
into important details, but experiences of using the method in more projects is still needed for better validation.
It seems that the underlying reason are the deeper discussions at the core of the structured scenarios. 
As the structure forced us to identify and then clarify important 
\emph{AECO} unknowns as soon as possible,
it made apparent which parts of the AECO procedure are still unclear.

\textbf{Advantages of ubiquitous language}.
A choice we made for the structured scenarios was to use BIM (and its open standard, IFC) as 
ubiquitous language (see Section~\ref{subsec:ubiquituous-language}).
This meant that we could use terms that was well defined from a software development perspective, 
but also something that was well known by many of the AECO professionals as BIM is used 
in a large share of construction projects, and a lot of today's AECO software tools and 
collaboration practices support it.
It might be fuzzy to talk about a ``named 3D area'' on the construction site, 
but we instead used \texttt{IfcZone} and that was clearly understood. 
In addition, \texttt{IfcZone} is exactly what one can require to be included in the IFC files 
that will be used as some of the inputs in the software tools that we will develop. 
We also chose to use IFC terms for concepts that we are not certain that we will IFC format for, 
because we wanted to take advantage of the clear definition existing in the IFC schema. 
One example for this is \texttt{IfcTask}.
Using this we know that it is a task, that it has a start and end time, 
that it is part of a workflow and that it can be related to a specific set of building elements. 
Yet another example is \texttt{IfcActor}, since that is a person, it can belong to an organization, 
and it can be responsible for a task.

On the other hand, the alternative approach lacked a clear terminology and consequently often missed
to define and (re-)use the concepts as explicitly (see Figure~\ref{fig:forecast-schedule}).

\begin{figure}
    \begin{center}
        \includegraphics[scale=0.25]{IDEF0_drawing_Forecast_schedule}
    \end{center}
    \captionof{figure}{%
    A ``black box'' describing a scenario ``Forecast schedule'' created using the alternative approach.
    We omit the list of requirements for readability.
    The scenario lacked precise definitions of the concepts and their properties.
    For example, what properties define a ``status of tasks'' or what does the concept
    ``schedule forecast'' entail.
    }
    \label{fig:forecast-schedule}
\end{figure}

\textbf{Re-usability}.
The ``black boxes'' of the alternative approach could obviously be reused among the different
scenarios and projects.
However, as they were not constrained by the dimensions of the solution space,
they tend to be tailored to the given problem at hand, where the levels of abstraction
move only along the axis of the \emph{given} problem.

Our approach primed the authors instead to think in abstractions along the three axes
of the solution space, thus making them reflect more on general abstractions.
For example, if we had to introduce helicopter deliveries, we can abstract the existing
scenario ``Truck Deliveries'' to a general one ``Deliveries'' 
by cutting out the device and person-specific details, and finally introducing
the ``Helicopter Delivery'' by replacing the truck-specific requirements in ``Truck Delivery''
with helicopter-specific requirements (see Figure~\ref{fig:level_marking}).
To the contrary, the corresponding scenario coming from the alternative approach 
based on ``black boxes'' would need more work as the details are not grouped by predefined 
levels of abstraction, but by arbitrary ones or even none, making them much harder to ``zoom out''
(see Figure~\ref{fig:IDEF0_schedule_machinery}).

\textbf{Judgement}.
When comparing the two approaches, both have their benefits. 
The alternative approach, brainstorming + IDEF0, is established and immediately practicable by both 
software professionals and AECO experts.
This makes it also democratic in larger groups since it scales very well in group size and 
heterogeneity.
The main benefits of our approach were the compact (but structured) notation and that 
it was possible to go much deeper at an earlier time.
Using IFC terms when having deep discussions with AECO experts was particularly beneficial and
brought about clearer communication.

